An NMF solution for the Flowgraphs case at the TTC 2013

Software systems are getting more and more complex. Model-driven engineering (MDE) offers ways to handle such increased complexity by lifting development to a higher level of abstraction. A key part in MDE are transformations that transform any given model into another. These transformations are used to generate all kinds of software artifacts from models. However, there is little consensus about the transformation tools. Thus, the Transformation Tool Contest (TTC) 2013 aims to compare different transformation engines. This is achieved through three different cases that have to be tackled. One of these cases is the Flowgraphs case. A solution has to transform a Java code model into a simplified version and has to derive control and data flow. This paper presents the solution for this case using NMF Transformations as transformation engine.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.5}{10.4204/EPTCS.135.5}}
\pdfoutput=1

